NL4DV: A Toolkit for Generating Analytic Specifications for Data Visualization from Natural Language Queries

Natural language interfaces (NLIs) have shown great promise for visual data analysis, allowing people to flexibly specify and interact with visualizations. However, developing visualization NLIs remains a challenging task, requiring low-level implementation of natural language processing (NLP) techniques as well as knowledge of visual analytic tasks and visualization design. We present NL4DV, a toolkit for natural language-driven data visualization. NL4DV is a Python package that takes as input a tabular dataset and a natural language query about that dataset. In response, the toolkit returns an analytic specification modeled as a JSON object containing data attributes, analytic tasks, and a list of Vega-Lite specifications relevant to the input query. In doing so, NL4DV aids visualization developers who may not have a background in NLP, enabling them to create new visualization NLIs or incorporate natural language input within their existing systems. We demonstrate NL4DV's usage and capabilities through four examples: 1) rendering visualizations using natural language in a Jupyter notebook, 2) developing a NLI to specify and edit Vega-Lite charts, 3) recreating data ambiguity widgets from the DataTone system, and 4) incorporating speech input to create a multimodal visualization system.

==> code-listings/mmplot-js-parsing-old.tex <==
\begin{listing}[t!]
\begin{minted}
[
baselinestretch=1,
fontsize=\scriptsize,
% xleftmargin=15pt,
xleftmargin=2.5pt,
% linenos,
breaklines,
style=manni
]
{javascript}

$.post("/analyzeQuery", {"query": query})
  .done(function (response_string) {
    let nl4dvResponse = JSON.parse(response_string);
    let attributeMap = nl4dvResponse['infoMap']['attributeMap'],       taskMap = nl4dvResponse['infoMap']['taskMap'];
    if(fingerPos==="AXIS"){
        let newAxisAttr = Object.keys(attributeMap)[0];
        // check which axis was pointed on and bind newAxisAttr to that axis.
    }else if(voiceTrigger==="MIC"){
        if("Filter" in taskMap){ // query includes a filter
            for(let taskObj of taskMap['Filter']['taskObjects'){
                for(let attr of taskObj['attributes']){
                    // check the attribute type, & parse the 'operator' and 'values' to apply requested filters
                }
            }
        }
    });
  
\end{minted}
\caption{\textcolor{black}{JavaScript code to parse NL4DV's output for supporting speech and multimodal interactions in \textsc{MMPlot} (Figure~\ref{fig:example-mmplot}-bottom).
}}
\label{listing:mmplot-js-parsing}
\end{listing}

% else if(voiceTrigger==="MIC"){
%         if(visList.length>0){ // query specifies a new chart
%             // parse the encodings from visList[0]['vlSpec'] to update the scatterplot using D3.js
%         }
%         if("Filter" in taskMap){ // query includes a filter
%             for(let taskObj in taskMap['Filter']){
%                 for(let attr of taskObj['attributes']){
%                     // check the attribute type & parse the 'operator' and 'values' to apply requested filters
%                 }
%             }
%         }
%     }

==> code-listings/test-listing.tex <==
\begin{listing}[t!]
\begin{minted}
[
baselinestretch=1,
fontsize=\footnotesize,
xleftmargin=15pt,
linenos,
breaklines,
style=manni
]
{javascript}

$.post("/analyzeQuery", {"query": query})
  .done(function (response_string) {
    let nl4dvResponse = JSON.parse(response_string);
    let attributeMap = nl4dvResponse['infoMap']['attributeMap'];
    for(let attr in attributeMap){
        if(attributeMap[attr]['isAmbiguous']===true){
            // add attr and items in attributeMap[attr]['ambiguity'] as options for a dropdown menu rendered under the DOM element corresponding to the attributeMap[attr]['queryPhrase'] in the input query string
        }
    }
  });
  
\end{minted}
\caption{\textcolor{black}{JavaScript code used to parse NL4DV's output and generate attribute-level ambiguity widgets in Figure~\ref{fig:example-datatone}.
Note that this example only covers attribute-level ambiguity but a similar logic is used to iterate over the \variable{taskMap} when creating data value-level ambiguities during filter tasks.
}}
\label{listing:test}
\end{listing}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/01-introduction.tex <==
% \firstsection{Introduction}
% \maketitle
\section{\arjun{Introduction (Original)}}

% \begin{itemize}
%     \item NLIs are becoming popular, developing these is difficult if you're a novice, (maybe) repetitive if you're an expert.
%     \item Example (maybe go with one explicit and one implicit)
%     \item NL4DV helps by doing x, y, z (show in context of example)
%     \item In this paper, we describe how NL4DV works and present XX sample use cases demonstrating its application in the context of data analysis and visualization system development.
%     \item In summary, our contributions are twofold:
%     \begin{itemize}
%         \item Formalization of visualization-related concepts from natural language queries. Specifically, data attributes, their corresponding data values, \& analytic tasks.
%         \item A toolkit NL4DV implementing this formalization. Examples demonstrating the application of the toolkit in different scenarios including A, B, and C.
%     \end{itemize}
% \end{itemize}

Natural language interfaces (NLIs) for visualization are becoming increasingly popular in both academic research (e.g.,~\cite{gao2015datatone,setlur2016eviza,hoque2018applying,srinivasan2018orko,yu2019flowsense}) as well as commercial software~\cite{mspowerbi,tableauaskdata}.
At a high-level, visualization NLIs allow people to pose data-related queries and generate visualizations relevant to those queries.
% In doing so, these interfaces show promise in helping novice users of visualization tools better analyze their data and for supporting rapid visual analysis.
To generate visualizations from natural language (NL) queries, NLIs first model the input query in terms of \textit{data attributes} and \textit{low-level analytic tasks}~\cite{amar2005low,chen2009toward} (e.g., filter, correlation, trend).
Using this information, the systems then determine which visualizations are most suited to respond to the input query. 
While NLIs provide flexibility in posing data-related questions, inherent characteristics of NL such as ambiguity and underspecification make inferring relevant information from NL queries a challenging task.

Consider the spectrum of queries in Figure~\ref{fig:teaser} issued to create visualizations in the context of an IMDb movies dataset
% \footnote{\arjun{Link to movies dataset}}
with different attributes including the {\small{\faHashtag}}~Worldwide Gross, {\small{\faFont}}~Genre, and {\small{\faCalendar}}~Release Year, among others (for consistency, we use this movies dataset for examples throughout this paper).
% \footnote{For consistency, we use this IMDb movies dataset as a running example in this paper. Note, however, that NL4DV is not preconfigured for specific datasets and can be used to query any tabular dataset provided in a CSV or JSON format.}.
The query \textit{``Create a histogram showing distribution of IMDB ratings"} (Figure~\ref{fig:teaser}a) explicitly refers to a data attribute (\textit{IMDB Rating}), a low-level analytic task (\textit{Distribution}), and requests a specific visualization type (\textit{Histogram}).
% \john{This is an ideal situation as the user has been very explicit and clear about all the components of their query.}
This is an ideal interpretation scenario from a system standpoint since the query explicitly lists all components required to generate a visualization.
On the other hand, the second query \textit{``Show average gross across genres for the science fiction and fantasy movies"} (Figure~\ref{fig:teaser}b) does not explicitly state the visualization type or the attribute \textit{Creative Type}.
Instead, it explicitly references the attributes \textit{Worldwide Gross} and \textit{Genre} through `gross' and `genres', and implicitly refers to the \textit{Creative Type} through the values `science fiction' and `fantasy'.
Furthermore, by specifying data values for the \textit{Creative Type} attribute and the word `average,' the query also mentions two intended analytic tasks: \textit{Filtering} and computing \textit{Derived Values}, respectively.
This second query is more challenging since it requires the system to implicitly infer one of the attributes and then determine the visualization type based on the identified attributes and tasks.
Finally, the third query \textit{``Visualize rating and budget"} (Figure~\ref{fig:teaser}c) is even more challenging to interpret since it neither explicitly states the desired visualization type nor the intended analytic task.
Furthermore, while it explicitly references one attribute (\textit{Production Budget} through `budget'), the reference to the second attribute is ambiguous (`rating' can map to \textit{IMDB Rating}, \textit{Content Rating}, or \textit{Rotten Tomatoes Rating}).
%\john{Queries like this begin to show the many challenges in providing NL input to data visualization systems.}

To accommodate such query variations, visualization NLIs employ sophisticated natural language processing (NLP) techniques (e.g., part-of-speech tagging, dependency parsing) to identify relevant information from the query and build upon visualization concepts (e.g.~analytic tasks) and design principles (e.g.~choosing graphical encodings based on attribute types) to generate appropriate visualizations.
For example, for the query in Figure~\ref{fig:teaser}b, after detecting the data attributes and analytic tasks, a visualization NLI should select a visualization (e.g.~bar chart) that is well-suited to support the task of displaying \textit{Derived Values} (average) for \textit{Worldwide Gross} (a {\small{\faHashtag}} quantitative attribute) across different \textit{Genre}s (a {\small{\faFont}} nominal attribute).
Similarly, in the scenario in Figure~\ref{fig:teaser}c, a NLI must first detect ambiguities in the input query attributes, determine the visualizations suited to present those attribute combinations (e.g.~\textit{scatterplot} for two quantitative attributes), and ultimately infer the analytic tasks based on those attributes and visualizations (e.g.~a scatterplot may imply the user is interested in finding \textit{correlations}).

To implement visualization NLIs, visualization system developers (henceforth, developers) currently need to possess knowledge of NLP techniques (to handle variations in queries), visualization design (to select most suited representations based on attributes and tasks), and visualization rendering and graphical user interface (GUI) tools to create the system interface.
Although there exist numerous resources to support GUI and visualization design (e.g., D3.js~\cite{bostock2011d3}, Vega-Lite~\cite{satyanarayan2016vega}), developers currently need to implement custom NLP modules to interpret NL queries and determine appropriate visualizations based on that interpretation.
However, for developers without experience with NLP techniques and toolkits (e.g., NLTK~\cite{loper2002nltk}, spaCy~\cite{honnibal2017spacy}), implementing this pipeline is non-trivial, requiring developers to spend significant time and effort in learning and implementing different NLP techniques.

To support prototyping NLIs for data visualization and aid developers who may not have a background in NLP, we present the \textit{Natural Language-Driven Data Visualization} (\textit{NL4DV}) toolkit.
Implemented as a Python package, NL4DV takes as input an NL query about a tabular dataset, and returns data attributes and analytic tasks inferred from the query as well as an ordered list of Vega-Lite specifications relevant to the input query.
In doing so, NL4DV abstracts out the core task of interpreting NL queries and also provides task-based visualization recommendation as plug-and-play functionality.
Using NL4DV, developers can create new visualization NLIs as well as incorporate NL querying capabilities into their existing visualization systems.

In summary, we make the following contributions:
\begin{itemize}
    \item We describe NL4DV's design goals and implementation, discussing how the toolkit infers data attributes, analytic tasks, and visualization specifications from NL queries and formalizes them into a JSON-based analytic specification that can be programmatically parsed to develop NLIs for data visualization.
    \item We showcase NL4DV's representative usage through exemplary scenarios demonstrating how the toolkit can help implement visualization NLIs from scratch, incorporate NL input into an existing visualization system, and support visualization specification in data science programming environments.
    % \arjun{(Shorten second one depending on user study results.)}
\end{itemize}
To support development of future systems, we also provide NL4DV and the described applications as open-source software (\arjun{\textit{link-to-review-repo}}).

% \arjun{
% Terminology consistency checks:
% \begin{itemize}
%     \item Query/utterance/command
%     \item rendering engine/library/toolkit
%     \item user/developer/designer
%     \item parse; process; interpret;
%     \item phrase/substring; token;
% \end{itemize}
% }

% \arpit{
% \begin{itemize}
%     % \item ++Motivation for the problem
%     % \item A SNEAK PEEK like: are you a developer/analyst/data scientist? have a dataset? want quick visual insight and no time to code? import nl4dv, initialize it with data, run an NL query, and bam! here's your viz could be a game changer as everyone who sees this for the first time is impressed.
%     % \item - - Use Cases: Can articulate (or make clear) the point that the toolkit's software architecture is like use-what-you-want: attributes, tasks and/or visualizations.
%     % \item Thought: Can create types of users like vis developers (only vis), nlp developers (only nlp), full stack developers (both nl+vis), data scientists (domain), business analysts (lil domain + lil tech + mostly management), Teachers (teach vis toolks like vega) and see how (if) NL4DV can be used to help each one of them.
% \end{itemize}
% }

==> sections/xx-evaluation.tex <==
\section{Performance Evaluation \arjun{[Needed?]}}

\begin{itemize}
        % \item \textbf{Strategy 1:} We have a collection of aprox.~50-70 queries corresponding to different visualizations for the superstore and movies datasets.
        % \textbf{Will report:} Overall accuracy + response time of executing collected queries with NL4DV.
        \item Two part study (30 min sessions, 10-12 participants): 1) Participants try to recreate 5-7 given charts with NL, and 2) Open-ended queries within the Vega-Lite editor application. Participants respond with a likert scale on if the recommended visualizations met their expectations. 
        \textbf{Will report:} Overall accuracy + execution time for collected queries; Distribution of participant ratings.
        % \item \textbf{Strategy 2:} Include a figure with 4-6 charts along with queries that work/do not work for specifying those charts.
\end{itemize}

==> sections/xx-limitations.tex <==
\section{\remove{Limitations and Future Work}}

% \begin{itemize}
%     \item More vis types \& tasks (e.g., compare, time series, QA)
%     \item Long term evaluation and usage
%     \item Cagatay's new semantic type detection to improve datatype recog. 
%     \item Supporting units (e.g., 100M)
%     \item Semantic enrichment (connecting to knowledge bases like WolframAlpha to determine what a `large' earthquake is)
%     \item \arpit{Thresholds (e.g. 0.8) for attribute similarity) are heuristic based.}
% \end{itemize}

\noindent\remove{
\contenttheme{Supporting other visualizations and tasks.}
In this initial version of NL4DV, we focus on supporting NL-based specification of basic visualizations such as bar charts, line charts, and scatterplots, among others in the context of tabular datasets.
Going forward, we will extend the toolkit to support additional visualization types including maps and networks.
Besides visualizations, we will also extend the set of analytic tasks inferred by NL4DV to support other tasks such as comparisons and finding outliers, enabling more robust querying and visualization specification.
While NL4DV currently allows overriding its default attribute type interpretations, we are also looking into incorporating recent semantic data type detection models (e.g.,~\mbox{\cite{zhang2019sato,hulsebos2019sherlock}}) within NL4DV directly.
Finally, expanding beyond visualization specification, another area for development is adding support for other capabilities such as question answering~\mbox{\cite{kim2020answering}} and formatting visualizations through NL~\mbox{\cite{srinivasan2020interweaving}}.
}

\noindent\remove{
\contenttheme{Improving query interpretation.}
The thresholds for matching query phrases to the lexicon and the dependency parsing rules are currently derived from sample queries and implementations of prior systems~\mbox{\cite{gao2015datatone,setlur2016eviza,hoque2018applying,yu2019flowsense}}.
Although deriving metrics from prior work provides a preliminary level of validation and supports replication, an important area for future work is to collect labeled data on utterances people use to specify visualizations.
Such datasets can allow leveraging ML techniques to develop more robust parsers that are inherently aligned with people's natural utterances.
Another area for improvement along these lines is to connect NL4DV to knowledge bases like WolframAlpha~\mbox{\cite{wolframalpha}} to semantically understand words in the input query.
Incorporating such connections can help resolve vague predicates for data values (e.g., `large', `expensive', `near')~\mbox{\cite{setlur2016eviza,setlur2019inferencing}} and may also reduce the need for developers to manually configure attribute aliases.
}

\noindent\remove{
\contenttheme{Longitudinal User Study.}
% Mention student projects + potential use by start-ups \& consultation firms.
We have tested NL4DV by querying it against tabular datasets containing between 300-6000 rows and up to 15 attributes.
We currently showcase NL4DV's capabilities through sample queries (additional queries are provided as supplementary material) and by illustrating applications developed using NL4DV.
However, effectively assessing the toolkit's value deems a more longitudinal study incorporating feedback from both visualization and NLP developers.
Such a study will help assess the practical usability of the toolkit (both from an API design and scalability standpoint), highlight potential issues, and understand the breadth of possible applications.
}
